Distributed Path Compression for Piecewise Linear Morse-Smale Segmentations and Connected Components

This paper describes the adaptation of a well-scaling parallel algorithm for computing Morse-Smale segmentations based on path compression to a distributed computational setting. Additionally, we extend the algorithm to efficiently compute connected components in distributed structured and unstructured grids, based either on the connectivity of the underlying mesh or a feature mask. Our implementation is seamlessly integrated with the distributed extension of the Topology ToolKit (TTK), ensuring robust performance and scalability. To demonstrate the practicality and efficiency of our algorithms, we conducted a series of scaling experiments on large-scale datasets, with sizes of up to 4096^3 vertices on up to 64 nodes and 768 cores.

==> figures/speedup_1024.tex <==
% This file was created with tikzplotlib v0.10.1.

\newcommand{\ssscaleX}{0.6}
\newcommand{\ssscaleY}{0.6}


\tikzstyle{spEdgeR}=[red, line width=0.25mm,opacity=1]
\tikzstyle{spEdgeB}=[blue, line width=0.25mm,opacity=0.8]
\tikzstyle{spEdgeG}=[gray, line width=0.25mm,opacity=0.8]

\hspace*{-1.6em}%
\begin{tikzpicture}

\definecolor{brown1672968}{RGB}{167,29,68}
\definecolor{darkcyan26118156}{RGB}{26,118,156}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{groupplot}[group style={group size=2 by 1,horizontal sep=2.5em}]
\nextgroupplot[
log basis x={2},
log basis y={2},
tick align=outside,
tick pos=left,
% title={Speedup},
% ylabel={Speedup},
x grid style={darkgray176,opacity=0.2, dashed},
xlabel={\#Nodes},
xmajorgrids,
xmin=1, xmax=64,
xmode=log,
xtick style={color=black},
y grid style={darkgray176,opacity=0.2, dashed},
ymajorgrids,
ymin=0, ymax=50,
ymode=log,
ytick style={color=black},
log ticks with fixed point,
xscale=\ssscaleX,yscale=\ssscaleY
]
\coordinate (c1) at (rel axis cs:0,1);
\addplot [spEdgeG] % vtk
table {%
1.0 1.0
2.0 1.4853626615847357
4.0 3.4620740091567925
8.0 9.129524148377568
16.0 17.224760389673616
32.0 30.357354859452276
64.0 47.328386641319774
};
\addplot [spEdgeR] % implicit cc
table {%
1.0 1.0
2.0 1.0795975971629153
4.0 2.5307018039925353
8.0 5.578072312754141
16.0 12.294065934065934
32.0 23.454088050314464
64.0 30.94771784232365
};
%\addplot [spEdgeB] % pc 
%table {%
%1.0 1.0
%2.0 0.538006814870658
%4.0 4.45095876777656
%8.0 6.911568024596464
%16.0 5.568460490463215
%32.0 4.485657986630749
%64.0 3.582022069075409
%};

\addplot [gray, dash pattern=on 3.7pt off 1.6pt]
table {%
1 1
2 2
4 4
8 8
16 16
32 32
64 64
};

\nextgroupplot[
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176,opacity=0.2, dashed},
xlabel={\#Nodes},
% ylabel={Parallel Efficiency},
% title={Parallel Efficiency},
xmajorgrids,
xmin=1, xmax=64,
xmode=log,
xtick style={color=black},
log ticks with fixed point,
y grid style={darkgray176,opacity=0.2, dashed},
ymajorgrids,
ymin=0, ymax=1.2,
ytick style={color=black},
% legend to name=legend,
% legend style={legend columns=2},
xscale=\ssscaleX,yscale=\ssscaleY
]
\coordinate (c2) at (rel axis cs:1,1);
% \addlegendentry{Extreem}
% \addlegendentry{PPP}
\addplot [spEdgeG] % vtk
table {%
1.0 1.0
2.0 0.7426813307923679
4.0 0.8655185022891981
8.0 1.141190518547196
16.0 1.076547524354601
32.0 0.9486673393578836
64.0 0.7395060412706215
};
\addplot [spEdgeR] % implicit cc
table {%
1.0 1.0
2.0 0.5397987985814576
4.0 0.6326754509981338
8.0 0.6972590390942677
16.0 0.7683791208791209
32.0 0.732940251572327
64.0 0.48355809128630706
};
%\addplot [spEdgeB] % pc
%table {%
%%1.0 1.0
%2.0 0.269003407435329
%4.0 1.11273969194414
%8.0 0.863946003074558
%%16.0 0.34802878065395093
%32.0 0.14017681208221092
%64.0 0.05596909482930327
%};
\end{groupplot}
    % \coordinate (c3) at ($(c1)!.5!(c2)$);
    % \coordinate (c4) at ($(c1)!.25!(c2)$);
    % \coordinate (c5) at ($(c1)!.75!(c2)$);
    % \coordinate (c4) at ;
    % \coordinate (c5) at (3,3);
    % \coordinate (c5) at (current bounding box.east);
    \node[above] at (2,3.4) {\textbf{Speedup}};
    \node[above] at (7,3.4) {\textbf{Parallel Efficiency}};
    % \node[above] at (c5) {Parallel Efficiency};
    % \coordinate (c3) at ($(c1)!.5!(c2)$);
    % \node[below] at (c3 |- current bounding box.south)
      % {\pgfplotslegendfromname{legend}};

\end{tikzpicture}


==> figures/speedup_2048.tex <==
% This file was created with tikzplotlib v0.10.1.

\newcommand{\ssscaleX}{0.6}
\newcommand{\ssscaleY}{0.6}


\tikzstyle{spEdgeR}=[red, line width=0.25mm,opacity=1]
\tikzstyle{spEdgeB}=[blue, line width=0.25mm,opacity=0.8]
\tikzstyle{spEdgeG}=[gray, line width=0.25mm,opacity=0.8]

\hspace*{-1.6em}%
\begin{tikzpicture}

\definecolor{brown1672968}{RGB}{167,29,68}
\definecolor{darkcyan26118156}{RGB}{26,118,156}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{gray}{RGB}{128,128,128}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{groupplot}[group style={group size=2 by 1,horizontal sep=2.5em}]
\nextgroupplot[
log basis x={2},
log basis y={2},
tick align=outside,
tick pos=left,
% title={Speedup},
% ylabel={Speedup},
x grid style={darkgray176,opacity=0.2, dashed},
xlabel={\#Nodes},
xmajorgrids,
xmin=1, xmax=64,
xmode=log,
xtick style={color=black},
y grid style={darkgray176,opacity=0.2, dashed},
ymajorgrids,
ymin=0, ymax=50,
ymode=log,
ytick style={color=black},
log ticks with fixed point,
xscale=\ssscaleX,yscale=\ssscaleY
]
\coordinate (c1) at (rel axis cs:0,1);
\addplot [spEdgeG] % vtk
table {%
1.0 1.0
2.0 1.9218817151621301
4.0 3.8430153127998588
8.0 7.570263861907543
16.0 14.74899316192058
32.0 27.52582464151619
64.0 50.32910708942333
};
\addplot [spEdgeR] % implicit cc
table {%
1.0 1.0
2.0 0.7307972574608326
4.0 2.4949960986531874
8.0 4.006177822373681
16.0 8.849892366218732
32.0 16.714687279252278
64.0 26.3987119899182
};

\addplot [gray, dash pattern=on 3.7pt off 1.6pt]
table {%
1 1
2 2
4 4
8 8
16 16
32 32
64 64
};

\nextgroupplot[
log basis x={2},
tick align=outside,
tick pos=left,
x grid style={darkgray176,opacity=0.2, dashed},
xlabel={\#Nodes},
% ylabel={Parallel Efficiency},
% title={Parallel Efficiency},
xmajorgrids,
xmin=1, xmax=64,
xmode=log,
xtick style={color=black},
log ticks with fixed point,
y grid style={darkgray176,opacity=0.2, dashed},
ymajorgrids,
ymin=0, ymax=1.2,
ytick style={color=black},
% legend to name=legend,
% legend style={legend columns=2},
xscale=\ssscaleX,yscale=\ssscaleY
]
\coordinate (c2) at (rel axis cs:1,1);
% \addlegendentry{Extreem}
% \addlegendentry{PPP}
\addplot [spEdgeG] % vtk
table {%
1.0 1.0
2.0 0.9609408575810651
4.0 0.9607538281999647
8.0 0.9462829827384429
16.0 0.9218120726200363
32.0 0.860182020047381
64.0 0.7863922982722396
};
\addplot [spEdgeR] % implicit cc
table {%
1.0 1.0
2.0 0.3653986287304163
4.0 0.6237490246632968
8.0 0.5007722277967102
16.0 0.5531182728886708
32.0 0.5223339774766337
64.0 0.4124798748424719
};
\end{groupplot}
    % \coordinate (c3) at ($(c1)!.5!(c2)$);
    % \coordinate (c4) at ($(c1)!.25!(c2)$);
    % \coordinate (c5) at ($(c1)!.75!(c2)$);
    % \coordinate (c4) at ;
    % \coordinate (c5) at (3,3);
    % \coordinate (c5) at (current bounding box.east);
    \node[above] at (2,3.4) {\textbf{Speedup}};
    \node[above] at (7,3.4) {\textbf{Parallel Efficiency}};
    % \node[above] at (c5) {Parallel Efficiency};
    % \coordinate (c3) at ($(c1)!.5!(c2)$);
    % \node[below] at (c3 |- current bounding box.south)
      % {\pgfplotslegendfromname{legend}};

\end{tikzpicture}


==> tables/overview_pc.tex <==

\begin{table*}[htb]
    \centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c | r !\lv r !\lv r !\lv r !\lv r !\lv r !\lv r}
\textbf{Size in \#Vertices }                           &                            \textbf{1N} &                            \textbf{2N} &                            \textbf{4N} &                            \textbf{8N}  &                            \textbf{16N}  &                            \textbf{32N}  &                            \textbf{64N}  \\
\midrule
$512^3$ & 11.291 & 20.629 & 1.468 & 2.440 & 3.687 & 4.875 & 6.785 \\


\lh
$1024^3$ & 86.044 & 167.134 & 17.417 & 13.010 & 16.148 & 20.046 & 25.103 \\

\lh
$2048^3$  & 905.872 & 2165.203 & 215.517 & 106.430 & 16 & 32 & 64 \\

\lh
$4096^3$   & 1 & 2 & 4 & 8 & 16 & 32 & 64 \\
\end{tabular}
}\vspace{0.5em}
\caption{
    Timing in seconds of Distributed Path Compression (DPC) run on Perlin Noise grouped by dataset size.
    The remaining columns show, per node count, the total runtime in seconds.
    For some datasets the computations ran out of memory or failed because of the previously described reasons and are therefore missing from the table.
}
    \label{tab:overview_pc}
\end{table*}


==> tables/perlin.tex <==
\begin{table}[]
    \centering
    \rowcolors{2}{gray!10}{white}
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l|rrrrrrr}
\toprule
\#Nodes & 1 & 2 & 4 & 8 & 16 & 32 & 64 \\
\midrule
Segmentation Computation & 1.477 & 5.453 & 0.798 & 2.435 & 5.900 & 10.452 & 25.414 \\
            \midrule
            \midrule

Implicit CC & 0.604 & 1.542 & 0.931 & 1.034 & 1.098 & 1.312 & 1.615 \\
Explicit CC & 0.010 & 0.886 & 0.819 & 1.048 & - & - & - \\
VTK CC & 0.730 & 0.813 & 0.832 & 0.968 & 1.031 & 1.241 & 1.361 \\
\bottomrule
\end{tabular}

    }
    \caption{Timing for Weak Scaling experiments based on Perlin Noise, generated at increasing sizes, starting from $256^3$ vertices and doubling with every doubled node count, up to $1024^3$ vertices. Algorithms marked with \emph{-} could not be run due to memory constraints.}
    \label{tab:perlin}
\end{table}



==> tables/perlin_2048.tex <==
\begin{table}[]
    \centering
    \rowcolors{2}{gray!10}{white}
    \resizebox{\columnwidth}{!}{%
\begin{tabular}{l|rrrrrrr}
\toprule
\#Nodes & 1 & 2 & 4 & 8 & 16 & 32 & 64 \\
\midrule
Implicit CC & 237.242 & 402.772 & 111.073 & 68.752 & 29.125 & 15.188 & 8.912 \\
VTK CC & 671.906 & 349.608 & 174.838 & 88.756 & 45.556 & 24.410 & 13.350 \\
\bottomrule
\end{tabular}

    }
    \caption{Timing for the strong scaling experiments based on Perlin Noise at a grid size of $2048^3$ vertices.}
    \label{tab:perlin_2048}
\end{table}

==> tables/perlin_strong.tex <==
\begin{table}[]
    \centering
    \rowcolors{2}{gray!10}{white}
    \resizebox{\columnwidth}{!}{%
     \begin{tabular}{l|rrrrr}
\toprule
\#Nodes & 4 & 8 & 16 & 32 & 64 \\
\midrule
Segmentation Computation & 11.356 & 13.963 & 16.799 & 20.309 & 25.473 \\
Implicit CC & 24.236 & 8.023 & 3.888 & 2.250 & 1.619 \\
VTK CC & 14.601 & 7.086 & 3.756 & 2.131 & 1.367 \\
\bottomrule
\end{tabular}

    }
    \caption{Timing for the strong scaling experiments based on Perlin Noise at a grid size of $1024^3$ vertices.}
    \label{tab:perlin_strong}
\end{table}


